Quantum Advantage with Sign-Free Proofs: An Oracle Separation between $\mathsf{StoqMA}$ and $\mathsf{MA}$

Several landmark oracle results (FOCS 2000, FOCS 2025, STOC 2026) establish strict separations along the chain $\mathsf{MA} \subseteq \mathsf{QCMA} \subseteq \mathsf{QMA}$, showing that quantum verification and quantum witnesses can each provide additional power over classical proof systems. These separations, however, use substantial coherent quantum computation, often through the quantum Fourier transform. We prove that a minimal quantum resource already suffices to outperform every classical verifier. Namely, we show the separation $$\mathsf{MA} \subsetneq \mathsf{StoqMA}$$ relative to a classical oracle. The class $\mathsf{StoqMA}$, introduced by Bravyi, Bessen, and Terhal (arXiv 2006), restricts the verifier to classical reversible computation, followed by a single Hadamard-basis measurement. Its power is closely tied to the complexity of stoquastic Hamiltonians, a sign-problem-free and seemingly more tractable class of quantum Hamiltonians. Our separating problem is to determine whether a sparse high-girth graph, given via an adjacency-list oracle, has a large or small Perron--Frobenius eigenvalue. This amounts to a ground-energy estimation task for a related stoquastic Hamiltonian. Our construction builds on a line of work on graph exploration problems with exponential quantum speedups, from welded trees (STOC 2003) to recent constructions (STOC 2021, arXiv 2026).

==> Figures/no-graph.tex <==
% Right-hand closure panel (TikZ picture fragment; not standalone).
% Requires \usepackage{tikz} in the paper preamble.
\definecolor{RBaseTeal}{HTML}{0D7A80}
\definecolor{RTreeLavender}{HTML}{A89BD0}
\definecolor{RTreeCharcoal}{HTML}{292733}
\definecolor{RVertexRed}{HTML}{E63232}
\definecolor{RMarkedRing}{HTML}{C43B42}
\definecolor{RClosureFill}{HTML}{FFF4D6}
\definecolor{RClosureOutline}{HTML}{D3B56F}
\definecolor{RBackgroundTeal}{HTML}{F0F7F7} % lighter green

% Fan-shaped tree. #1 attachment, #2 orientation, #3 edge colour,
% #4 scale, #5 colour of vertices. The same topology is used for each instance.
\newcommand{\closureFanTree}[5]{%
  \begin{scope}[shift={#1},rotate=#2,scale=#4]
    \tikzset{closurefanedge/.style={draw=#3,line width=0.48pt,line cap=round,line join=round}}
    \draw[closurefanedge] (0,0) -- (1,0);
    \node[circle,fill=#5,draw=#5,inner sep=0pt,minimum size=1.9pt] at (1,0) {};
    \foreach \theta in {-50,-25,0,25,50}{%
      \pgfmathsetmacro{\bx}{1+3.2*cos(\theta)}%
      \pgfmathsetmacro{\by}{3.2*sin(\theta)}%
      \draw[closurefanedge] (1,0) -- (\bx,\by);
      \node[circle,fill=#5,draw=#5,inner sep=0pt,minimum size=1.7pt] at (\bx,\by) {};
      \foreach \delta in {-10,-5,0,5,10}{%
        \pgfmathsetmacro{\la}{\theta+\delta}%
        \pgfmathsetmacro{\lx}{1+6.2*cos(\la)}%
        \pgfmathsetmacro{\ly}{6.2*sin(\la)}%
        \draw[closurefanedge] (\bx,\by) -- (\lx,\ly);
        \node[circle,fill=#5,draw=#5,inner sep=0pt,minimum size=1.6pt] at (\lx,\ly) {};
      }%
    }%
  \end{scope}%
}

% Fan tree rooted directly at the end of a long connector.
% Unlike \closureFanTree, this has NO extra stem edge or extra root vertex:
% the coordinate supplied in #1 is the root, which branches immediately.
% #1 root coordinate, #2 rotation, #3 edge colour, #4 scale, #5 vertex colour.
\newcommand{\closureFanTreeRoot}[5]{%
  \begin{scope}[shift={#1},rotate=#2,scale=#4]
    \tikzset{closurefanrootedge/.style={draw=#3,line width=0.48pt,line cap=round,line join=round}}
    \node[circle,fill=#5,draw=#5,inner sep=0pt,minimum size=1.9pt] at (0,0) {};
    \foreach \theta in {-50,-25,0,25,50}{%
      \pgfmathsetmacro{\bx}{3.2*cos(\theta)}%
      \pgfmathsetmacro{\by}{3.2*sin(\theta)}%
      \draw[closurefanrootedge] (0,0) -- (\bx,\by);
      \node[circle,fill=#5,draw=#5,inner sep=0pt,minimum size=1.7pt] at (\bx,\by) {};
      \foreach \delta in {-10,-5,0,5,10}{%
        \pgfmathsetmacro{\la}{\theta+\delta}%
        \pgfmathsetmacro{\lx}{6.2*cos(\la)}%
        \pgfmathsetmacro{\ly}{6.2*sin(\la)}%
        % Soft translucent red halos identify the leaves as boundary vertices.
        \fill[RVertexRed,opacity=0.16] (\lx,\ly) circle (0.34);
        \draw[closurefanrootedge] (\bx,\by) -- (\lx,\ly);
        \node[circle,fill=#5,draw=#5,inner sep=0pt,minimum size=1.6pt] at (\lx,\ly) {};
      }%
    }%
  \end{scope}%
}

% Purple fan tree with an independently adjustable edge from the host vertex to the tree root.
% #1 host coordinate, #2 orientation, #3 edge colour, #4 fan scale,
% #5 tree-vertex colour, #6 length of the host-to-root edge (in cm).
\newcommand{\closureFanTreeLongStem}[6]{%
  \begin{scope}[shift={#1},rotate=#2]
    \draw[draw=#3,line width=0.48pt,line cap=round,line join=round] (0,0) -- (#6,0);
    \begin{scope}[shift={(#6,0)},scale=#4]
      \node[circle,fill=#5,draw=#5,inner sep=0pt,minimum size=1.9pt] at (0,0) {};
      \foreach \theta in {-50,-25,0,25,50}{%
        \pgfmathsetmacro{\bx}{3.2*cos(\theta)}%
        \pgfmathsetmacro{\by}{3.2*sin(\theta)}%
        \draw[draw=#3,line width=0.48pt,line cap=round,line join=round] (0,0) -- (\bx,\by);
        \node[circle,fill=#5,draw=#5,inner sep=0pt,minimum size=1.7pt] at (\bx,\by) {};
        \foreach \delta in {-10,-5,0,5,10}{%
          \pgfmathsetmacro{\la}{\theta+\delta}%
          \pgfmathsetmacro{\lx}{6.2*cos(\la)}%
          \pgfmathsetmacro{\ly}{6.2*sin(\la)}%
          \draw[draw=#3,line width=0.48pt,line cap=round,line join=round] (\bx,\by) -- (\lx,\ly);
          \node[circle,fill=#5,draw=#5,inner sep=0pt,minimum size=1.6pt] at (\lx,\ly) {};
        }%
      }%
    \end{scope}%
  \end{scope}%
}

% Five short open edge stubs around a specified outward direction.
% #1 is a coordinate, #2 is the central angle in degrees.
\newcommand{\closureStubFan}[2]{%
  \foreach \sa in {-20,-10,0,10,20}{%
    \draw[RBaseTeal,line width=0.43pt] #1 -- ++({0.30*cos(#2+\sa)},{0.30*sin(#2+\sa)});
  }%
}

\begin{tikzpicture}[x=1cm,y=1cm,line cap=round,line join=round]
  % Ambient graph and closure region: two circles, with translucent yellow fill.
  \fill[RBackgroundTeal] (0,0) circle (4.55);
  \draw[RBaseTeal,line width=0.8pt] (0,0) circle (4.55);
  \fill[RClosureFill,fill opacity=0.64] (0,0) circle (2.72);
  \draw[RClosureOutline,line width=0.75pt] (0,0) circle (2.72);

  % Core structure: four extended straight paths whose intersections delimit
  % a square. Every extension and every attached branch lies inside the yellow circle.
  % First draw a translucent thick overlay over ALL core-path and branch edges.
  \tikzset{corehighlight/.style={draw=RBaseTeal,line width=3.6pt,opacity=0.17,line cap=round,line join=round}}
  \draw[corehighlight] (-2.15,1.05) -- (-1.60,1.05) -- (-1.05,1.05) -- (-0.55,1.05) -- (0,1.05) -- (0.55,1.05) -- (1.05,1.05) -- (1.60,1.05) -- (2.15,1.05);
  \draw[corehighlight] (-2.15,-1.05) -- (-1.60,-1.05) -- (-1.05,-1.05) -- (-0.55,-1.05) -- (0,-1.05) -- (0.55,-1.05) -- (1.05,-1.05) -- (1.60,-1.05) -- (2.15,-1.05);
  \draw[corehighlight] (-1.05,-1.05) -- (-1.05,-0.55) -- (-1.05,0) -- (-1.05,0.55) -- (-1.05,1.05) -- (-1.05,1.60) -- (-1.05,2.15);
  \draw[corehighlight] (1.05,-1.05) -- (1.05,-0.55) -- (1.05,0) -- (1.05,0.55) -- (1.05,1.05) -- (1.05,1.60) -- (1.05,2.15);
  % Exactly one downward extension vertex is retained at each lower square-side corner.
  \draw[corehighlight] (-1.05,-1.05) -- (-1.05,-1.45);
  \draw[corehighlight] (1.05,-1.05) -- (1.05,-1.45);
  % Branches are tree-like and extend OUTWARD from the square; they do not form cycles.
  \draw[corehighlight] (-0.55,1.05) -- (-0.55,1.48) -- (-0.82,1.88);
  \draw[corehighlight] (-0.55,1.48) -- (-0.23,1.88);
  \draw[corehighlight] (0.55,1.05) -- (0.55,1.48) -- (0.23,1.88);
  \draw[corehighlight] (0.55,1.48) -- (0.87,1.88);
  \draw[corehighlight] (-1.05,0) -- (-1.50,0) -- (-1.92,0.28);
  \draw[corehighlight] (-1.50,0) -- (-1.92,-0.30);
  \draw[corehighlight] (1.05,0) -- (1.50,0) -- (1.92,0.28);
  \draw[corehighlight] (1.50,0) -- (1.92,-0.30);

  % The same paths and branches, now in the normal thin base-graph edge colour.
  \tikzset{coreedge/.style={draw=RBaseTeal,line width=0.58pt,line cap=round,line join=round}}
  \draw[coreedge] (-2.15,1.05) -- (-1.60,1.05) -- (-1.05,1.05) -- (-0.55,1.05) -- (0,1.05) -- (0.55,1.05) -- (1.05,1.05) -- (1.60,1.05) -- (2.15,1.05);
  \draw[coreedge] (-2.15,-1.05) -- (-1.60,-1.05) -- (-1.05,-1.05) -- (-0.55,-1.05) -- (0,-1.05) -- (0.55,-1.05) -- (1.05,-1.05) -- (1.60,-1.05) -- (2.15,-1.05);
  \draw[coreedge] (-1.05,-1.05) -- (-1.05,-0.55) -- (-1.05,0) -- (-1.05,0.55) -- (-1.05,1.05) -- (-1.05,1.60) -- (-1.05,2.15);
  \draw[coreedge] (1.05,-1.05) -- (1.05,-0.55) -- (1.05,0) -- (1.05,0.55) -- (1.05,1.05) -- (1.05,1.60) -- (1.05,2.15);
  \draw[coreedge] (-1.05,-1.05) -- (-1.05,-1.45);
  \draw[coreedge] (1.05,-1.05) -- (1.05,-1.45);
  \draw[coreedge] (-0.55,1.05) -- (-0.55,1.48) -- (-0.82,1.88);
  \draw[coreedge] (-0.55,1.48) -- (-0.23,1.88);
  \draw[coreedge] (0.55,1.05) -- (0.55,1.48) -- (0.23,1.88);
  \draw[coreedge] (0.55,1.48) -- (0.87,1.88);
  \draw[coreedge] (-1.05,0) -- (-1.50,0) -- (-1.92,0.28);
  \draw[coreedge] (-1.50,0) -- (-1.92,-0.30);
  \draw[coreedge] (1.05,0) -- (1.50,0) -- (1.92,0.28);
  \draw[coreedge] (1.50,0) -- (1.92,-0.30);

  % Five open stubs at every vertex of the four extended paths (length 0.30 cm so they clear marked rings).
  % Top and bottom rows: outward is up and down, respectively.
  \foreach \x in {-2.15,-1.60,0,1.60,2.15}{\closureStubFan{(\x,1.05)}{90}}
  \closureStubFan{(-0.55,1.05)}{125}
  \closureStubFan{(0.55,1.05)}{55}
  % Corners use a radial fan; these are also marked vertices.
  \closureStubFan{(-1.05,1.05)}{135}
  \closureStubFan{(1.05,1.05)}{45}
  \foreach \x in {-2.15,-1.60,0,1.60,2.15}{\closureStubFan{(\x,-1.05)}{270}}
  \closureStubFan{(-1.05,-1.05)}{225}
  \closureStubFan{(1.05,-1.05)}{315}
  % Selected lower-edge vertices: four open stubs each, angled into the green region; the fifth outward edge is the long tree connector.
  \foreach \a in {-130,-120,-110,-100}{\draw[RBaseTeal,line width=0.43pt] (-0.55,-1.05) -- ++({0.30*cos(\a)},{0.30*sin(\a)});}
  \foreach \a in {-80,-70,-60,-50}{\draw[RBaseTeal,line width=0.43pt] (0.55,-1.05) -- ++({0.30*cos(\a)},{0.30*sin(\a)});}
  % Top extensions and branch attachments have outward stub fans as well.
  \foreach \y in {-0.55,0.55,1.60,2.15}{\closureStubFan{(-1.05,\y)}{180}\closureStubFan{(1.05,\y)}{0}}
  \closureStubFan{(-1.05,-1.45)}{270}
  \closureStubFan{(1.05,-1.45)}{270}
  % The two side branch roots replace the ordinary side fan by a slightly oblique fan,
  % avoiding overlap with the actual branch edge.
  % (Overdrawn directions at y=0 are visually suppressed by the central vertex markers.)
  \closureStubFan{(-1.05,0)}{210}
  \closureStubFan{(1.05,0)}{-30}

  % Stubs along the outward branch trees, all five per branch vertex.
  \closureStubFan{(-0.55,1.48)}{90}
  \closureStubFan{(-0.82,1.88)}{90}
  \closureStubFan{(-0.23,1.88)}{90}
  \closureStubFan{(0.55,1.48)}{90}
  \closureStubFan{(0.23,1.88)}{90}
  \closureStubFan{(0.87,1.88)}{90}
  \closureStubFan{(-1.50,0)}{180}
  \closureStubFan{(-1.92,0.28)}{145}
  \closureStubFan{(-1.92,-0.30)}{215}
  \closureStubFan{(1.50,0)}{0}
  \closureStubFan{(1.92,0.28)}{35}
  \closureStubFan{(1.92,-0.30)}{-35}

  % Two long connectors leave the selected bottom-edge vertices and end directly
  % at the roots of the large trees. The roots branch immediately (no extra stem
  % or duplicate vertex). Removing the lower side-path vertices above keeps each
  % connector clear of the square network. The smaller trees remain fully inside the green boundary.
  \draw[RBaseTeal,line width=0.62pt] (-0.55,-1.05) -- (-1.25,-2.56);
  \draw[RBaseTeal,line width=0.62pt] (0.55,-1.05) -- (1.25,-2.56);
  \closureFanTreeRoot{(-1.25,-2.56)}{-125}{RBaseTeal}{0.24}{RVertexRed}
  \closureFanTreeRoot{(1.25,-2.56)}{-55}{RBaseTeal}{0.24}{RVertexRed}

  % External annotation: the arrow points directly to the highlighted boundary leaves.
  \node[font=\small,text=black,anchor=west] at (4.18,-2.16) {\emph{boundary}};
  \draw[->,draw=black,line width=0.65pt] (4.08,-2.31) -- (2.69,-2.49);

  % Directional continuation marks around the green region (eight orientations).
  \node[text=RBaseTeal,font=\small,rotate=90]  at (0,3.82) {$\cdot\;\cdot\;\cdot$};
  \node[text=RBaseTeal,font=\small,rotate=45]  at (2.72,2.72) {$\cdot\;\cdot\;\cdot$};
  \node[text=RBaseTeal,font=\small,rotate=0]   at (3.78,0) {$\cdot\;\cdot\;\cdot$};
  \node[text=RBaseTeal,font=\small,rotate=-45] at (3.15,-1.90) {$\cdot\;\cdot\;\cdot$};
  \node[text=RBaseTeal,font=\small,rotate=90]  at (0,-3.95) {$\cdot\;\cdot\;\cdot$};
  \node[text=RBaseTeal,font=\small,rotate=45]  at (-3.15,-1.90) {$\cdot\;\cdot\;\cdot$};
  \node[text=RBaseTeal,font=\small,rotate=0]   at (-3.78,0) {$\cdot\;\cdot\;\cdot$};
  \node[text=RBaseTeal,font=\small,rotate=-45] at (-2.72,2.72) {$\cdot\;\cdot\;\cdot$};

  % Red vertices of the square paths and all outward branches.
  \foreach \x in {-2.15,-1.60,-1.05,-0.55,0,0.55,1.05,1.60,2.15}{%
    \node[circle,fill=RVertexRed,draw=RVertexRed,inner sep=0pt,minimum size=2.2pt] at (\x,1.05) {};
    \node[circle,fill=RVertexRed,draw=RVertexRed,inner sep=0pt,minimum size=2.2pt] at (\x,-1.05) {};
  }
  \foreach \y in {-1.05,-0.55,0,0.55,1.05,1.60,2.15}{%
    \node[circle,fill=RVertexRed,draw=RVertexRed,inner sep=0pt,minimum size=2.2pt] at (-1.05,\y) {};
    \node[circle,fill=RVertexRed,draw=RVertexRed,inner sep=0pt,minimum size=2.2pt] at (1.05,\y) {};
  }
  \foreach \x/\y in {-0.55/1.48,-0.82/1.88,-0.23/1.88,0.55/1.48,0.23/1.88,0.87/1.88,-1.50/0,-1.92/0.28,-1.92/-0.30,1.50/0,1.92/0.28,1.92/-0.30,-1.05/-1.45,1.05/-1.45}{%
    \node[circle,fill=RVertexRed,draw=RVertexRed,inner sep=0pt,minimum size=2.2pt] at (\x,\y) {};
  }

  % Exactly five marked vertices on the square network: only the left large-tree attachment is ringed; the right attachment is not.
  \foreach \x/\y in {-2.15/1.05,1.05/2.15,1.05/0.55,-0.55/-1.05,2.15/-1.05}{%
    \draw[RMarkedRing,line width=0.85pt] (\x,\y) circle (0.15);
  }

  % Three lavender decorations: at a marked square vertex, on a base-graph tree in green,
  % and at another square-network vertex. The attached vertices retain their red base-graph colour.
  \closureFanTreeLongStem{(-1.05,1.05)}{-45}{RTreeLavender}{0.085}{RTreeCharcoal}{0.22}
  \closureFanTreeLongStem{(1.051,-3.302)}{180}{RTreeLavender}{0.060}{RTreeCharcoal}{0.22}
  % This is the theta=0 first-level vertex on the left teal fan tree.
  \closureFanTreeLongStem{(-1.051,-3.302)}{0}{RTreeLavender}{0.060}{RTreeCharcoal}{0.18}
  \closureFanTreeLongStem{(1.05,0.55)}{180}{RTreeLavender}{0.085}{RTreeCharcoal}{0.22}
\end{tikzpicture}
